Graph Neural PDE Solvers with Conservation and Similarity-Equivariance

Utilizing machine learning to address partial differential equations (PDEs) presents significant challenges due to the diversity of spatial domains and their corresponding state configurations, which complicates the task of encompassing all potential scenarios through data-driven methodologies alone. Moreover, there are legitimate concerns regarding the generalization and reliability of such approaches, as they often overlook inherent physical constraints. In response to these challenges, this study introduces a novel machine-learning architecture that is highly generalizable and adheres to conservation laws and physical symmetries, thereby ensuring greater reliability. The foundation of this architecture is graph neural networks (GNNs), which are adept at accommodating a variety of shapes and forms. Additionally, we explore the parallels between GNNs and traditional numerical solvers, facilitating a seamless integration of conservative principles and symmetries into machine learning models. Our findings from experiments demonstrate that the model's inclusion of physical laws significantly enhances its generalizability, i.e., no significant accuracy degradation for unseen spatial domains while other models degrade. The code is available at https://github.com/yellowshippo/fluxgnn-icml2024.

==> Makefile <==
# Change NAME accordingly
NAME = fluxgnn
# DIFF_REF = bb806e391654b4d70b86c2b9636ee770736353d2

TEX = pdflatex
# TEX = pdflatex -shell-escape -interaction=nonstopmode -file-line-error
DVI = dvipdfmx
PRE =  $(TEX) -ini -job-name="preamble" "&pdflatex preamble.tex\dump"
BIB = bibtex


one: $(NAME).tex
	$(TEX) $(NAME).tex
	pdffonts $(NAME).pdf
	open $(NAME).pdf

embed: pdf
	/opt/homebrew/bin/gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOutputFile=$(NAME).converted.pdf $(NAME).pdf
	mv $(NAME).converted.pdf $(NAME).pdf
	pdffonts $(NAME).pdf


all: pdf view

pdf: $(NAME).pdf

# diff:
# 	cp iclr2021_conference.bbl iclr2021_conference-diffad0f7d35.bbl
# 	yes | latexdiff-vc -s COLOR --disable-auto-mbox --exclude-textcmd="textit,footnote,section,subsection" --graphics-markup=0 --math-markup=0 --git -r $(DIFF_REF) $(NAME).tex
# 	# yes | latexdiff-vc --append-textcmd=scalebox --git -r $(DIFF_REF) $(NAME).tex
# 	$(TEX) $(NAME)-diff$(DIFF_REF).tex
# 	open $(NAME)-diff$(DIFF_REF).pdf

view:
	pdffonts $(NAME).pdf
	open $(NAME).pdf

clean:
	$(RM) \
		$(NAME).pdf $(NAME).dvi $(NAME).aux $(NAME).log $(NAME).out \
		$(NAME).bbl $(NAME).blg

$(NAME).pdf: $(NAME).tex $(NAME).bib
	$(TEX) $(NAME).tex
	bibtex $(NAME)
	$(TEX) $(NAME).tex
	$(TEX) $(NAME).tex

bib:
	bibtex $(NAME)

figure: figure.tex
	$(TEX) figure.tex
	open figure.pdf

